The "Non-Musk Effect" at Twitter

Elon Musk has long been known to significantly impact Wall Street through his controversial statements and actions, particularly through his own use of social media. An innovator and visionary entrepreneur, Musk is often considered a poster boy for all entrepreneurs worldwide. It is, thus, interesting to examine the effect that Musk might have on Main Street, i.e., on the social media activity of other entrepreneurs. In this research, we study and quantify this "Musk Effect," i.e., the impact of Musk's recent and highly publicized acquisition of Twitter on the tweeting activity of entrepreneurs. Using a dataset consisting of 9.94 million actual tweets from 47,190 self-declared entrepreneurs from seven English-speaking countries (US, Australia, New Zealand, UK, Canada, South Africa, and Ireland) spanning 71 weeks and encompassing the entire period from the rumor that Musk may buy Twitter till the completion of the acquisition, we find that only about 2.5% of the entrepreneurs display a significant change in their tweeting behavior over the time. We believe that our study is one of the first works to examine the effect of Musk's acquisition of Twitter on the actual tweeting behavior of Twitter users (entrepreneurs). By quantifying the impact of the Musk Effect on Main Street, we provide a comparison with the effect Musk's actions have on Wall Street. Finally, our systematic identification of the characteristics of entrepreneurs most affected by the Musk Effect has practical implications for academics and practitioners alike.

==> leaning_by_cohort.tex <==
\begin{tabular}{lrlr}
  \hline
Group&Leaning&Group&Leaning\\ \hline
3&-0.0030 & 8&-0.0022\\
7&-0.0027 & 5&-0.0021\\
6&-0.0027 & 1&-0.0004\\
4&-0.0026 & 2& 0.0006\\\hline
\end{tabular}

